PQC Migration of IPsec: Reliable Composite Key Sharing Mechanisms in IKEv2

The threat of quantum computers breaking classical cryptographic is accelerating the adoption of quantum- resistant cryptographic algorithms. Several government agencies have set a tight time-line for upgradation of all system to support post quantum cryptographs. We study post-quantum migration of IPSec protocols and their impact on network performance. The large key lengths in Post-Quantum Cryptography (PQC) cannot fit in a single IP packet leading to IP fragmentation. This can cause failure of security associations and degrade performance of IKEv2 under poor network conditions. To tackle this problem, we study a new key- sharing mechanism for IKEv2 and evaluate its performance. Unlike current hybrid key-sharing approaches, which send the classical and quantum keys sequentially over UDP or TCP (as in RFC 9370), the new approach concatenates them into a single composite key and transport them over TCP to ensure a reliable handshake. We implement and benchmark the new composite key-sharing handshake mechanism against existing hybrid algorithms that use either UDP or TCP. Extensive experiments under various network conditions demonstrate that the new approach significantly improves handshake time and energy consumption by avoiding the severe retransmission penalties of the Hybrid handshake mechanism. At 1% packet loss, the handshake time of composite key sharing mechanism is better by atleast 20% than hybrid mechanisms, and the improve- ment get better with higher packet loss reaching 30% at 10% packet loss. Energy consumption follows the same pattern achieving reduction of 29% at 10% packet loss

==> sections/06f_cpu_cycles.tex <==
%% sections/06f_cpu_cycles.tex — §6.7 CPU Cycles

\subsection{CPU Cycles}
\label{sec:results:cycles}

The raw cryptographic cost of post-quantum key exchange is negligible relative
to IKEv2 protocol overhead. Table~\ref{tab:cycles} reports cycles and energy
per handshake at ideal conditions with ML-DSA-44 authentication.
The baseline is Crv25519$+$ML-KEM-768\,(H/UDP) at approximately 40.2\,M cycles.

\begin{table}[htb]
\centering
\setlength{\tabcolsep}{4pt}
\setlength{\arrayrulewidth}{0.4pt}
{\footnotesize
\begin{tabular}{|l|r|r|r|}
\hline
\rowcolor{tableheader}
\textbf{\color{white}Algorithm} &
\textbf{\color{white}Cycles\,(M)} &
\textbf{\color{white}Energy\,(mJ)} &
\textbf{\color{white}$\Delta$ Cycles} \\
\hline
\rowcolor{compositecol!15}Crv25519$\Vert$768\,(C/TCP)   & 43.4 & 347 & $+$3.2\,M\;($+$8\%) \\
\rowcolor{compositecol!15}ECP-256$\Vert$768\,(C/TCP)    & 44.2 & 352 & $+$4.0\,M\;($+$10\%) \\
\rowcolor{compositecol!15}ECP-384$\Vert$1024\,(C/TCP)   & 56.5 & 431 & $+$16.3\,M\;($+$41\%) \\
\hline
\rowcolor{hybridcol!15}Crv25519$+$768\,(H)   & 44.7 & 359 & $+$4.5\,M\;($+$11\%) \\
\rowcolor{hybridcol!15}ECP-256$+$768\,(H)    & 45.5 & 361 & $+$5.3\,M\;($+$13\%) \\
\rowcolor{hybridcol!15}ECP-384$+$1024\,(H)   & 58.6 & 446 & $+$18.4\,M\;($+$46\%) \\
\hline
\rowcolor{gray!10}\multicolumn{4}{|l|}{\textit{Baseline: Crv25519$+$768\,H/UDP\,$\approx$\,40.2\,M cycles, 323\,mJ}} \\
\hline
\end{tabular}
}
\caption{CPU cycles and energy per handshake at ideal conditions (ML-DSA-44 auth).
  $\Delta$ relative to Crv25519$+$ML-KEM-768\,(H) baseline~$\approx$~40.2\,M cycles.
  H/TCP and H/UDP share the same cryptographic cost; transport choice affects only
  handshake duration, not per-round-trip computation.}
\label{tab:cycles}
\end{table}

ML-KEM adds only 3--5\,M cycles (7--11\%) over the classical Curve25519 baseline.
Authentication dominates the computational overhead far more than key exchange:
ML-DSA-44 adds approximately 4.5\,M cycles per handshake; ML-DSA-65 adds
7.8\,M cycles; ML-DSA-87 adds 11.2\,M cycles. These increments are strictly
additive and independent of both the key exchange algorithm and network conditions.

